DyMU: Dynamic Merging and Virtual Unmerging for Efficient VLMs

We present DyMU, an efficient, training-free framework that dynamically reduces the computational burden of vision-language models (VLMs) while maintaining high task performance. Our approach comprises two key components. First, Dynamic Token Merging (DToMe) reduces the number of visual token embeddings by merging similar tokens based on image complexity, addressing the inherent inefficiency of fixed-length outputs in vision transformers. Second, Virtual Token Unmerging (VTU) simulates the expected token sequence for large language models (LLMs) by efficiently reconstructing the attention dynamics of a full sequence, thus preserving the downstream performance without additional fine-tuning. Unlike previous approaches, our method dynamically adapts token compression to the content of the image and operates completely training-free, making it readily applicable to most state-of-the-art VLM architectures. Extensive experiments on image and video understanding tasks demonstrate that DyMU can reduce the average visual token count by 32%-85% while achieving comparable performance to full-length models across diverse VLM architectures, including the recently popularized AnyRes-based visual encoders. Furthermore, through qualitative analyses, we demonstrate that DToMe effectively adapts token reduction based on image complexity and, unlike existing systems, provides users more control over computational costs. Project page: https://mikewangwzhl.github.io/dymu/.

==> sections/0_abstract.tex <==


\begin{abstract}




\vspace{-10pt}

We present \ours, an efficient, training-free framework that dynamically reduces the computational burden of vision-language models (VLMs) while maintaining high task performance. Our approach comprises two key components. First, Dynamic Token Merging (\dtome) reduces the number of visual token embeddings by merging similar tokens based on image complexity, addressing the inherent inefficiency of fixed-length outputs in vision transformers. Second, Virtual Token Unmerging (VTU) simulates the expected token sequence for large language models (LLMs) by efficiently reconstructing the attention dynamics of a full sequence, thus preserving the downstream performance without additional fine-tuning. Unlike previous approaches, our method dynamically adapts token compression to the content of the image and operates completely training-free, making it readily applicable to most state-of-the-art VLM architectures. Extensive experiments on image and video understanding tasks, demonstrate that \ours can reduce the average visual token count by 32\%-85\% while achieving comparable performance to full-length models, across diverse VLM architectures, including the recently popularized AnyRes-based visual encoders. Furthermore, through qualitative analyses we demonstrate that \dtome effectively adapts token reduction based on image complexity, and unlike existing systems, provides users more control over computational costs.


\end{abstract}


==> sections/1_intro.tex <==

\vspace{-12pt}
\section{Introduction}
\label{sec:intro}


Recent large vision-language models (VLMs) have demonstrated breakthroughs in computer vision tasks such as image captioning~\cite{mscoco_caption}, open-vocabulary object detection~\cite{gupta2019lvis}, visual-question answering~\cite{vqav2} and OCR~\cite{ocrvqa} by leveraging the reasoning capabilities of large language models (LLMs) to enhance visual understanding. 
Most state-of-the-art Vision-Language Models (VLMs) follow a common approach: a visual encoder extracts features from images or videos and projects them into the same embedding space as textual features. These visual embeddings are then processed by LLMs alongside textual query features, enabling complex understanding and reasoning tasks while directly benefiting from advancements in LLM capabilities. 

As expected, the quality of the final predictions from the LLM relies heavily on the richness of the visual features and the amount of semantic detail captured by the encoder. Consequently, research has focused on improving visual encoders to extract increasingly fine-grained features, leading to architectures that can capture intricate details.
However, this level of detail comes at a cost --- the computational burden during training and inference.

To process high-resolution images while preserving fine-grained details, modern visual encoders generate a large number of tokenized representations. Furthermore, state-of-the-art VLMs like LLaVA-OneVision~\cite{llava-ov} and Qwen-2.5VL~\cite{qwen25vl} use vision transformers (ViTs) that scale the number of tokens with the resolution of the image or number of frames in videos. For example, the visual encoder in LLaVA-OneVision would produce 9477 tokens for an image of 1280$\times$960 resolution.
In contrast, the number of tokens in the textual queries for vision tasks is relatively low. On common benchmarks that represent real world use cases, textual queries often consist of just a few tokens, e.g., $\sim$24 on MME~\cite{fu2023mme}. This stark contrast highlights that the computational burden of processing vision tasks generally arises primarily from the large number of visual tokens.

We first make an interesting observation: in current visual encoders, the number of tokens generated for an image does not depend on the content of the image. In Figure~\ref{fig:teaser}, we illustrate this with some examples --- a CLIP~\cite{clip} representation leads to the same embedding size on a blank image with a small circle and on a complex scene depicting buildings, vehicles and people. In contrast, textual tokens are more closely tied to the amount of content conveyed --- more words are required to describe more information.
An average sentence length in English is around 15–20 words~\cite{francis79browncorpus}, meaning that \textit{regardless of the content of the image}, the language model in LLaVA-OneVision~\cite{llava-ov} has to process the equivalent of 400-500 sentences for each high-resolution image.

In this work, we propose \textbf{Dynamic Merging and Virtual Unmerging (\ours)}, which comprises two key methods for modifying existing pre-trained Vision-Language Models (VLMs). First, we introduce Dynamic Token Merging (Sec~\ref{subsec:batchtome}), which allows the \textit{visual encoder} to generate variable-length token sequences based on the complexity of the image. Second, we present Virtual Token Unmerging (Sec~\ref{subsec:tokexpansion}), enabling the \textit{LLM decoder} to process shorter dynamic visual token sequences while efficiently approximating the full-length sequence. Crucially, we demonstrate that both of these modifications \textit{do not require additional fine-tuning of the pre-trained VLM}. Furthermore, Dynamic Token Merging is compatible with any Vision Transformer (ViT)-based visual encoder, and Virtual Token Unmerging can be applied to any LLM that utilizes Rotary Position Embedding (RoPE)~\cite{rope}.

We show that VLMs modified with our methods can maintain the performance of the full model while reducing the average token count by 32\%-85\% (see Sec~\ref{sec:quant}). In addition to improving efficiency, our approach offers users greater control over token costs compared to existing systems (e.g., GPT-4o), which incur a fixed token count per image based solely on resolution. In Sec~\ref{sec:qualitative}, we demonstrate example applications on how the number of visual tokens can be further reduced by combining \ours with pre-processing tools such as background removal, object detection, etc. Through comprehensive quantitative experiments (Sec~\ref{sec:quant}), we verify that our method works effectively across different VLM architectures, with varying pre-training strategies, visual encoders, and training datasets.



==> sections/2_method.tex <==

\input{figures/method_figure}

\section{Method}
\label{sec:method}

In this section, we present the main technical details of proposed method. In Section~\ref{subsec:batchtome}, we present our proposed Dynamic Token Merging (\dtome) --- a training-free method to dynamically reduce the number of output tokens by visual encoders based on the complexity of the image content. 
In Section~\ref{subsec:tokexpansion}, we introduce Virtual Token Unmerging (\vtu) --- an approach to process the reduced visual tokens through the language model while efficiently simulating the standard number of visual tokens. This method utilizes the tracked positions of the redundant tokens to recreate a full attention matrix of the original length. 

The combination of both methods is referred to as \ours, short for Dynamic Merging and Virtual Unmerging. We illustrate the core idea in Figure~\ref{fig:method}.
\ours can be applied to any VLM that uses transformer-based visual encoders and RoPE-based transformer language models. The proposed modifications to the architecture do not introduce any additional learnable parameters and most importantly, do not require any additional fine-tuning of the VLM.

\subsection{Dynamic Token Merging (\dtome)}
\label{subsec:batchtome}


Most recent large vision-language models (VLMs) use vision transformers (ViTs) like CLIP~\cite{clip} or SigLIP~\cite{siglip} to encode images into a sequence of visual tokens. For a fixed resolution input image, the ViT architecture always outputs the same number of token embeddings, leading to low efficiency in VLMs.
Our approach draws inspiration from ToMe\cite{tome}, a prior work which reduces the number of output tokens to a predefined fixed number. 
However, predefining the reduction ratio can still lead to a misalignment between the information of an image and the number of tokens needed for representing it. 

Here we propose Dynamic Token Merging (\dtome), an extension of ToMe that adaptively merges similar tokens in ViT layers, ensuring the output token count aligns with image complexity. \dtome merges tokens based on a similarity threshold while maintaining a record of merged tokens to ensure their influence is properly propagated through subsequent transformer layers. 
To find the thresholds, we propose a inference-only batch-level bipartite merging algorithm which leverages the natural variance of image complexity in randomly sampled images.


\paragraph{Identifying Redundant Tokens} Let us represent the output of the self-attention layer in the ViT layer $i$ as $x_{i}\in \mathbb{R}^{N_i\times D}$, where $N_i$ is the sequence length\footnote{For standard ViT without any merging, $N_i$ is constant across layers} and $D$ is the embedding dimension. Similarly, let the keys computed in the self-attention layer be represented by $k_i\in \mathbb{R}^{N_i\times D_k}$. In each transformer block, we apply an additional \dtome operator to $x_i$. Drawing inspiration from \cite{tome}, we follow a bipartite soft matching strategy to identify which tokens need to be merged. First, we divide the $N_i$ tokens into two sets (say $\mathbb{A}$ and $\mathbb{B}$) by assigning alternating tokens in sequence them. We then compute a bipartite assignment between the two sets of tokens by assigning token $t\in \mathbb{A}$ to $t_B = \textstyle\arg\max\limits_{n \in \mathbb{B}} (k_i[t]^T~k_i[n])$ (token with the most similar key). This gives us $|\mathbb{A}|$ edges with scores $\textstyle S_i[t] = (k_i[t]^T~k_i[t_B])$ for $t\in \mathbb{A}$. We then apply a threshold $\tau_i$ to retain edges $t\xrightarrow[]{} t_B$ where $S_i[t]>\tau_i$. Unlike \cite{tome}, this thresholding operation leads to a variable number of retained edges depending on the amount of redundancy demonstrated in the key embeddings $k_i$. We describe our approach for computing the thresholds below.

\paragraph{Tracking and Merging Tokens} For each token in the sequence, $x_{i}[t]$, we also track the set of positions of the tokens that have already been merged into it.  $\mathbf{P}_i[t]\subset \{1,2,\dots,N_1\}$. For each of the edges between chosen redundant tokens $t\xrightarrow[]{} t_B$, we compute merged token embeddings and the corresponding position sets as:

{\footnotesize
\vspace{-9pt}
\begin{align}
        x_i{\left[t_B\right]} &\xleftarrow{} \frac{x_i{\left[t\right]} \cdot |\mathbf{P}_i{\left[t\right]}| + x_i{\left[t_B\right]} \cdot |\mathbf{P}_i{\left[t_B\right]}|}{|\mathbf{P}_i{\left[t\right]}| + |\mathbf{P}_i{\left[t_B\right]}|} \\[10pt]
        \mathbf{P}_i{\left[t_B\right]} &\xleftarrow{} \mathbf{P}_i{\left[t_B\right]} \cup \mathbf{P}_i{\left[t\right]} \\[10pt]
        \mathbf{P}_i{\left[t\right]} &\xleftarrow{} \varnothing
\end{align}
}
Intuitively, the representation of token $t_B$ is updated to the average of $x_i[t_B]$ and $x_i[t]$, weighted by their corresponding merged position set sizes, $\mathbb{P}_i[t_B]$ and $\mathbf{P}_i[t]$. The token $t$ is then dropped since it has been merged with $t_B$, thereby reducing the token count in the next layer.

\paragraph{Finding Redundancy Thresholds} The layer-wise thresholds $\tau_i$ play a crucial role in determining how many tokens are merged. In order to determine the thresholds, we rely of statistics from a large dataset of images. First, we choose a hyper-parameter $r_i$ for each layer $i$ which represents the number of edges we expect to merge in a layer \textbf{\textit{on average across images of all complexities}}. The final output would then be expected to have an \textit{average} of $N-\sum r_i$ tokens. Using a dataset of images, we collect large batches of size $B$ which are used to perform forward computation through the layers of the ViT sequentially. For each layer, we compute the $B$ bipartite matching token edge score maps $S^{(b)}[t]$ where $b\in \{1, 2,\dots ,B\}$ as previously described. We then find the threshold $\tau_i$ as: 

{\footnotesize
\vspace{-7pt}
\begin{align}
\tau_i = \max \left\{ \tau \mid \sum^B_{b=1} \sum_{t\in \mathbb{A}^{(b)}} \mathbb{I}\left( S^{(b)}[t] > \tau \right) = B*r_i \right\}
\end{align}
}

In words, this finds the largest threshold such that $B*r_i$ tokens are merged across the batch of images. It is important to note that the number of tokens merged in each image will not necessarily be equal to $r_i$ but the \textit{average} number of tokens merged per image will be $r_i$. 
Intuitively, since the ranking of edges is over the entire batch, simpler images that have more redundant tokens will be merged more.
This process is done sequentially for each layer while only passing the remaining tokens to the next layer to obtain thresholds for every layer. We then average the layer-wise thresholds across several batches to ensure that they reflect the statistics across a diverse set of images. See Figure~\ref{fig:method} (left) for an illustration of the proposed batch-level threshold finding.

\paragraph{Size Weighted Self-attention} To ensure that the self-attention layers weigh each token based on the number of tokens that were previously merged into it, we adopt the idea of size-weighted self-attention from ToME\cite{tome} where the attention is computed as:

{\footnotesize
\vspace{-10pt}
\begin{align}
    \mathbf{A} &= \texttt{Softmax} \left(\frac{\mathbf{QK}^T}{\sqrt{d}} + \log \left[\begin{matrix} |\mathbb{P}_i[1]| \\ \vdots\\ |\mathbb{P}_i[N_i]| \end{matrix}\right]\right)
\end{align}
}










\subsection{Virtual Token Unmerging (\vtu)}
\label{subsec:tokexpansion}

The language model (LLM) in a pre-trained VLM is trained to operate on a fixed number of embeddings for each image\footnote{AnyRes\cite{llava-ov} leads to multiple fixed length embeddings}. When Dynamic Token Merging is applied to a visual encoder, this disrupts the optimized VLM and leads to a significant drop in performance (see Sec~\ref{sec:experiments}). 
In this section, we present an approach to circumvent this issue while still benefiting from processing fewer number of visual embeddings. 
Our proposed approach, \vtufull{} (\vtu), can be easily applied to any mainstream LLM that uses a RoPE~\cite{rope}-based transformer architecture. 

Consider the general case of a sequence of $N$ embeddings $e\in \mathbb{R}^{N\times D}$ of which only $N_\uniq<<N$ rows are unique. Let $e_\uniq\in \mathbb{R}^{N_\uniq\times D}$ be the unique embeddings and $M\in \{0,1\}^{N\times N_\uniq}$ be a mapping such that $e = M ~ e_\uniq$. Here $M$ is a sparse matrix with one-hot rows\footnote{Note that due to the sparsity of $M$, the time complexity of multiplying $MD, DM, M^TD, DM^T$ are all $O(NK)$ if $D$ is a dense matrix with dimensions $N\times K$ or $K\times M$.}. We now ask the question --- for various operators $f$ in an LLM, can we approximate $f(e)$ using some efficient function of $e_\uniq$ and $M$?

\paragraph{Sequence-independent Operators} 
For any operator $f$ that processes each sequence location independently, we can express 
$f(e)$ as $f(e) = M~ f(e_\uniq)$ by definition. 
This means that we only need to apply $f$ to the unique embeddings $e_\uniq$, significantly reducing computational cost while preserving the original outputs.
Many key components of modern LLMs fall into this category, including Linear layers, Activation functions (ReLU, GeLU, etc.), and Layer Normalization (along the embedding dimension $D$). 


\input{tables/main_result_sota}
\input{tables/siglip_results}

\subsubsection*{Virtual Unmerging for Self-Attention with RoPE}
A common layer in recent LLMs is the Self-Attention operation with Rotary Position Embedding (RoPE). Unlike sequence-independent operators, self-attention considers pairwise interactions between embeddings and assigns a unique position to each of the $N$ locations in $e$. Consequently, directly applying $f(e_\uniq)$ fails to capture the structure of $e$, generally leading to significant discrepancies in the output.  

To address this, we derive an efficient method to compute $f(e)$ while preserving the benefits of token reduction. The key insight is to reconstruct the self-attention matrix without explicitly expanding the token sequence. We leverage the linearity of the RoPE transformation to efficiently simulate the appropriate repetitions and the positions of the unique embeddings, significantly reducing computational overhead while maintaining consistency with the full sequence computation.  

Let $Q=W_q e$, $K=W_k e$ and $V=W_v e$ be the full query, key and value matrices. Similarly, $Q_\uniq,K_\uniq$ and $V_\uniq$ are the unique queries, keys and values satisfying the mapping $M$ defined above. The RoPE Self-Attention similarity matrix is computed as $A = \mathtt{RoPE}(Q)\mathtt{RoPE}(K)^T$.

For simplicity, let us consider the case where $D=2$, so that we can write $Q = [Q_1, Q_2]$ where $Q_1, Q_2\in \mathbb{R}^{N}$. We will follow a similar notation for all queries, keys and values.  This allows us to express each query and key as a complex number \textit{i.e.} $Q[n] = Q_1[n] + \mathbf{i} Q_2[n]$. Let $\boldsymbol{\theta}\in [0, 2\pi)^N$ be the rotation angle associated with each position for RoPE. For positions $n,m\in {1,2,\dots N}$, the RoPE-based similarity~\cite{rope} is defined as:

{\footnotesize
\vspace{-5pt}
\begin{align}
A[m,n] &= \text{Re}\big( ~~e^{i\boldsymbol{\theta[m]}}Q[m]  ~~~\overline{e^{i\boldsymbol{\theta[n]}}K[n]} ~~ \big)\\
\small  &= \text{Re}\big( ~~Q[m]\overline{K[n]}  ~~ e^{i(\boldsymbol{\theta}[m]-\boldsymbol{\theta}[n])} ~~\big)
\end{align}
}

\noindent where $\overline{x},\text{Re}(x)$ denote the complex conjugate and the real part of $x$ respectively. This can be expanded as:

{\scriptsize
\vspace{-5pt}
\begin{align}
\begin{aligned}
\label{eq:attention_entry}
A[m,n] &= (Q_1[m]K_1[n] + Q_2[m]K_2[n]) \cos(\boldsymbol{\theta}[m]-\boldsymbol{\theta}[n]) \\
&\quad + (Q_1[m]K_2[n] - Q_2[m]K_1[n]) \sin (\boldsymbol{\theta}[m]-\boldsymbol{\theta}[n])
\end{aligned}
\end{align}
}

We also have the trigonometric identities:

{\footnotesize
\vspace{-5pt}
\begin{align}
\begin{aligned}
\label{eq:trig_expansion}
\cos(\theta[m] – \theta[n]) = \cos (\theta[m]) \cos(\theta[n]) + \sin(\theta[m]) \sin(\theta[n])\\
\sin(\theta[m] – \theta[n]) = \sin (\theta[m]) \cos(\theta[n]) - \cos(\theta[m]) \sin(\theta[n])
\end{aligned}
\end{align}
}



Let $C=\mathtt{diag}(\cos(\boldsymbol{\theta})), S=\mathtt{diag}(\sin(\boldsymbol{\theta}))$. Using Eq ~\ref{eq:attention_entry} \& ~\ref{eq:trig_expansion}, the matrix form for self-attention similarities is:

{\footnotesize
\vspace{-10pt}
\begin{align}
\begin{aligned}
A &= C QK^{\top} C + S QK^{\top} S \notag + S (Q\times K^{\top})C -  C(Q\times K^{\top})S 
\end{aligned}
\end{align}
}

\noindent where {\small$QK^T = Q_1K_1^T + Q_2K_2^T,\; Q\times K^{\top} = Q_1K_2^{\top} - Q_2K_1^{\top}$}.
This formulation can be applied to queries and keys of any dimension $D$ by repeating this for the $(D/2)$ complex numbers obtained by dividing the representation into two parts. In practice, a different $\boldsymbol{\theta}$ is used for each of the $(D/2)$ components. 

Using this formulation and the mapping M, we can rewrite the attention matrix in terms of the unique queries and keys as:

{\footnotesize
\vspace{-10pt}
\begin{align}
\label{eq:expand_sim}
A &= C M Q_\text{un} K_\text{un}^{\top} M^{\top} C 
   + S M Q_\text{un} K_\text{un}^{\top} M^{\top} S \notag \\
  &\quad + S M (Q_\text{un} \times K_\text{un}^{\top}) M^{\top} C 
   - C M (Q_\text{un} \times K_\text{un}^{\top}) M^{\top} S
\end{align}
}


Observe {\small $CM, M^TC, SM, M^TS$} are highly sparse, each with at most $N$ non-zero entries. These matrices can also be pre-computed and reused across all self-attention layers. Computing $Q_\text{un} K_\text{un}^{\top}$ and $Q_\text{un}\times K_\text{un}^{\top}$ incurs an $O(N_\uniq^2)$ cost whereas the each of the other matrix multiplications in Eq~\ref{eq:expand_sim} can be efficiently computed using sparse matrix operations in $O(N N_\uniq)$.
We can then use the attention matrix to compute the final output of the layer as:

\begin{footnotesize}
\vspace{-5pt}
\begin{align}
f(e) = \mathtt{smax} ( \frac{A}{\sqrt{D}} ) V = [\mathtt{smax} ( \frac{A}{\sqrt{D}} ) M] V_\uniq \notag
\end{align}
\end{footnotesize}

Unfortunately, the output $f(e)\in \mathbb{R}^{N\times D}$ will not necessarily exhibit the same redundancy as $e$. This in turn means that the future self-attention layers cannot benefit from the efficiency of virtual token unmerging. In order to remedy this, before passing the output to the future layers, we re-introduce the redundancy by averaging the embeddings in the positions that were originally equal. We denote this \textit{re-merged} output by $f'(e_\uniq, M)$ which can be written as:

{\footnotesize
\vspace{-5pt}
\begin{align}
\label{eq:uniq_selfattn_out}
f'(e_\uniq, M) &= (M^{\top} M)^{-1} M^T f(e) \notag \\
&= (M^{\top} M)^{-1} M^T \mathtt{smax} ( \frac{A}{\sqrt{D}} ) V 
\end{align}
}

While the above averaging operation breaks the exactness of the future operations, we observe empirically (see Section~\ref{sec:experiments}) that this re-merging of tokens, that are known to be redundant, causes minimal drop in performance.  

\paragraph{Overall Efficiency} The computation of attention matrix $A$ incurs a cost of $O(N_{un}^2 D + N N_{un} D)$ (due to the $D/2$ components). Followed by the softmax and sparse matrix multiplications in Eq~\ref{eq:uniq_selfattn_out} which incur a cost of $O(N^2 + N_\uniq^2 D)$. Therefore, the overall complexity for RoPE Self-Attention with Virtual Token Unmerging is $O(N_\uniq N D)$. For comparison, the full RoPE Self-Attention on a sequence length of $N$ would be an $O(N^2 D)$ operation. Therefore, we see a linear improvement in efficiency as the number of redundant tokens increases.
























==> sections/3_experiments.tex <==

\section{Experiments}
\label{sec:experiments}

In this section, we present all the details of our implementation of the proposed method. We also present a comprehensive analysis demonstrating the practical benefits and efficacy of utilizing \ours with various VLMs, visual encoders and LLM architectures.

\subsection{Implementation Details}
\label{sec:implementation}
\paragraph{\dtomefull{}} For \dtome, we find layer-wise thresholds using a diverse dataset of 250k images sampled from the SFT instruction tuning data of LLaVA 1.5~\cite{llava15} comprising of images from MS-COCO~\cite{mscoco}, VisualGenome~\cite{visual_genome}, OCR-VQA~\cite{ocrvqa}, TextVQA~\cite{textvqa} and GQA~\cite{hudson2019gqa}. We also ablate the choice of image datasets in \S\ref{sec:quant}. In general, a sufficiently diverse image set suffices, and performance remains robust to dataset changes. 
Importantly, we only use the images to estimate the thresholds (in inference mode) and do not use the associated annotations or text in any way.

\paragraph{\ours variants} 
For each visual encoder in the experiments, including CLIP~\cite{clip}\footnote{CLIP version: openai/clip-vit-large-patch14-336} and SigLIP~\cite{siglip, siglipso400m}\footnote{SigLIP with LLaVA-1.5: timm/ViT-B-16-SigLIP-384}\footnote{SIgLIP version with LLaVA-OV: google/siglip-so400m-patch14-384}, we find thresholds for three variants of the encoder by choosing different \textit{average} number of tokens to drop ($r_i$) in each layer. We represent these variants by \textit{$\bullet$-low,$\bullet$-mid,$\bullet$-high} corresponding to the expected average number of tokens. 
We also explore different VLM backbones including fixed-resolution models, e.g., LLaVA 1.5~\cite{llava15} and any-resolution models, e.g., LLaVA-OneVision~\cite{llava-ov}.

\subsection{Quantitative Evaluation}
\label{sec:quant}
\paragraph{Comparing Visual Token Merging Methods for VLMs}

In order to evaluate efficacy of our approach, we compare against several existing methods that focus on reducing the number of tokens for VLMs. To the best of our knowledge, our proposed approach is the first to 1) enable varied number of visual tokens and 2) not require further fine-tuning of the VLM. Nevertheless, we compare to methods that are designed to reduce the number of tokens by a fixed length. In Table~\ref{tab:sota}, we present a quantitative evaluation of all methods applied to a pre-trained LLaVA 1.5~\cite{llava15} architecture on standard VLM benchmarks, including GQA~\cite{hudson2019gqa}, MMBench~\cite{liu2023mmbench}, MME~\cite{fu2023mme}, POPE~\cite{pope}, ScienceQA~\cite{scienceqa}, SEED-IMG~\cite{seed_bench}, TextVQA~\cite{textvqa}, MMVet~\cite{yu2023mmvet}, LLaVA-Bench~\cite{llava15}.
\ours achieves average performances of 97.7\%, 99.1\%, and 100.4\%, relative to the original pretrained model, while reducing the token number by 84.5\%, 66.1\%, and 31.6\%, respectively. \ours also outperforms previous training-free methods while enabling varied length output per instance.
When decreasing the token number, the largest drop happens in TextVQA, which fits our expectation as understanding visual text is highly sensitive to the spatial location of visual tokens, on which the token merging tend to break.


\input{tables/llava_ov_results}

\input{figures/complexity}

\input{figures/radar_vtu}


\paragraph{Compatibility with Different LLMs and Visual Encoders}
\ours can be seamlessly integrated into multiple variants of VLMs featuring different LLMs, visual encoders, and pretraining strategies. In Tables~\ref{tab:sota} and \ref{tab:siglip_results}, we demonstrate that \ours effectively maintains baseline performance when applied both CLIP~\cite{clip} to SigLIP~\cite{siglip} representations within the LLaVA 1.5 framework, using a Vicuna-7B~\cite{vicuna2023} LLM.

Furthermore, in Table~\ref{tab:llava_ov_results} we evaluate \ours on LLaVA-OneVision~\cite{llava-ov}, a recent Any-Resolution (AnyRes) model with SigLIP-so400M~\cite{siglipso400m} as visual encoder and Qwen2~\cite{yang2024qwen2technicalreport} as LLM backbone. AnyRes enables processing images of arbitrary resolutions by segmenting them into smaller regions and encoding each individually. Our results show that \ours remains compatible with this complex operation, preserving performance while dynamically reducing token counts.
Additionally, we extend our evaluation to video benchmarks using LLaVA-OneVision. 
By applying \ours to the visual encoder, we achieve a variable reduction in feature representations per frame while maintaining strong performance across benchmarks.



\paragraph{Image Complexity vs Number of Tokens} 
In Figure~\ref{fig:complexity} (left), we show how the number of tokens varies with image complexity. We quantify image complexity $C(I)$ by computing the JPEG compression ratio, i.e., $C(I) = \frac{S_{JPEG}(I)}{H\times W}$, where $S_{JPEG}$ is the size (in bytes) of the image $I$ after JPEG encoding, and $H,W$ are the original height and width.
For this experiment, we use CLIP-L/14-336 with \dtome\textit{-low} to encode images in the MME benchmark. We observe a strong correlation between the number of output tokens and image complexity, indicating that \dtome effectively preserves essential details in complex images while reducing redundancy in simpler ones. We include more qualitative visualizations in Appendix~\ref{app:vis_img_to_tok}.

\input{figures/pixmo_vs_llava}
\input{figures/qualitative}

\paragraph{Fixed vs Dynamic Token Reduction} In Figure~\ref{fig:complexity} (right), we categorize images into three bins based on their complexity scores, and compare the performance of ToMe (fixed-length token reduction) and \dtome on the MME benchmark. A key drawback of fixed token reduction is its inability to adapt to image complexity, leading to over-compression for complex images and under-compression for simpler ones. While our method outperforms ToMe across all complexity levels, we observe the most significant gains on complex images, where ToMe struggles due to an insufficient number of tokens.

\paragraph{Importance of \vtufull}
\vtu efficiently reconstructs the representation of a full visual token sequence from a reduced set of visual tokens
To demonstrate its impact, we compare LLaVA 1.5 variants with and without \vtu. 
In the latter, the LLM does not undergo any modifications and directly receives fewer tokens.
In Figure~\ref{fig:radar_vtu}, we evaluate this effect on two token reduction methods: ToMe~\cite{tome}, which produces fixed-length sequences, and \dtome (ours). Across both cases, we observe that applying \vtu significantly improves performance on 8 out of 9 benchmarks, demonstrating its effectiveness in preserving model capabilities despite token reduction.

\paragraph{Impact of Dataset for Threshold Finding} The \dtome thresholds  are computed using images from the LLaVA instruction tuning dataset. Here, we investigate the sensitivity of \dtome to the threshold estimation dataset. In Figure~\ref{fig:threshold_dataset}, we evaluate \ours-LLaVA 1.5  with \dtome thresholds estimated on the Pixmo-Cap~\cite{deitke2024molmo} image-captioning dataset. We observe a minimal performance change across all the benchmarks, highlighting the robustness of our method to dataset variation. 
Interestingly, we observe that the thresholds estimated using the Pixmo-Cap dataset lead to fewer tokens during inference on the benchmarks. We hypothesize that this is due to the domain shift between the Pixmo-Cap images and a more diverse LLaVA-instruct dataset which covers diverse real-world use cases.


\subsection{Qualitative Analysis}
\label{sec:qualitative}

\vspace{-1pt}
\paragraph{Visualizing Variable Visual Token Length} \dtome facilitates producing variable number of token embeddings for images based on complexity of the content. In Appendix Figure~\ref{fig:img_to_tok_grid}, we visualize the number of visual tokens for various images from nine benchmarks. For each benchmark, we present three images corresponding to the minimum, median, and maximum token numbers output by \ours-low. We observe a strong correlation, both within and across different benchmarks, between image complexity and the number of tokens retained by \ours.

\paragraph{Controllable Visual Token Length}
Dynamic Token Merging offers a key advantage over fixed token reduction methods: cost controllability. By dynamically adjusting the number of visual tokens based on image complexity, users gain direct control over the computational cost incurred per image. 
This flexibility allows flexible combination of visual reasoning tools with \ours to further boost efficiency while maintaining performance.
For instance, in Figure~\ref{fig:qualitative}, we show example applications of combining \ours with additional tools, i.e., background removal~\cite{RMBG14}, OCR~\cite{onnxtr2024}, and object detection~\cite{owlvit} models, to extract focused regions and further reduce token count.
Unlike existing VLMs, which impose a fixed token budget per image regardless of content, our method enables adaptive token allocation, ensuring that simpler regions consume fewer resources while more complex regions retain the necessary level of detail.


==> sections/4_related_work.tex <==
\section{Related Work}

\input{tables/comparison_w_prev_work}

\paragraph{Efficient Vision-Language Models}
Recent efforts in large vision-language models (VLMs) have primarily focused on reducing computational overhead during the pre-filling and VLM decoding phases. That is, given a full sequence of visual tokens from a visual encoder, such as CLIP, these approaches perform token pruning and merging~\cite{llava-prumerge, fast-v, xing2024pyramiddrop, zhang2024sparsevlm, dynamic-llava, dynamic_token_reduction, ye2024atp}, distillation~\cite{ye2024voco}, or resampling~\cite{llama-vid, MQT-LLAVA, li2024tokenpacker, llava_mini} to improve efficiency in either the projectors or the VLM decoder blocks.
However, we identify several key limitations: (1) Most existing methods, including all training-free approaches~\cite{fast-v, xing2024pyramiddrop, zhang2024sparsevlm} predefine a fixed compression ratio for any input image regardless of its complexity. While \cite{ye2024atp} proposed an adaptive token pruning framework that enables variable-length compression, it requires retraining the backbone VLM with additional modules. Such training can be costly or infeasible as mainstream VLMs rarely open-source their full training recipe and data. (2) All existing methods retain a frozen, fixed-length visual encoder, overlooking the potential for further efficiency improvements within the visual encoder itself.
In this work, we aim to explore a simple training-free algorithm for variable length visual token compression, which can be directly applied to cutting-edge VLM architectures including Any-Resolution models and RoPE embeddings.

\paragraph{Efficient Vision Transformers}
We also draw inspiration from a separate line of research~\cite{token_pooling, tome, wu2023ppt, Avit, adaptive_sparse_vit} aimed at improving the efficiency of Vision Transformers (ViTs) themselves, which is still the main go-to architecture for visual encoders~\cite{clip, siglip, oquab2023dinov2}. In particular, ToMe~\cite{tome} merges a predefined number of tokens within each ViT block using bipartite soft matching. However, the effectiveness of such methods in coordination with VLM backbones remains largely unexplored. Our experiments in \S\ref{sec:experiments} show that naively applying ToMe to visual encoders in pretrained VLMs results in a significant drop in performance. To address this issue, we further propose an efficient ``virtual unmerging'' algorithm to boost the performance of VLMs without training with the modified encoders that output reduced token numbers.





==> sections/5_conclusion.tex <==
\section{Conclusions and Future Work}
\vspace{-1pt}
In this work, we introduced \ours, the first training-free framework that dynamically reduces visual token counts in VLMs based on per-image complexity. \ours can be directly plugged into all mainstream VLMs that comprise ViT-based visual encoders and RoPE-based LLM backbones. Future work includes improving \ours's ability to preserve VLM performance on spatially sensitive tasks such as TextVQA~\cite{textvqa} and spatial reasoning. Additionally, exploring the extension of \ours to reduce temporal redundancy in videos is another promising direction.




